Aperiodic two-way transducers and FO-transductions

Deterministic two-way transducers on finite words have been shown by Engelfriet and Hoogeboom to have the same expressive power as MSO-transductions. We introduce a notion of aperiodicity for these transducers and we show that aperiodic transducers correspond exactly to FO-transductions. This lifts to transducers the classical equivalence for languages between FO-definability, recognition by aperiodic monoids and acceptance by counter-free automata.

==> macros.tex <==
\usepackage{stmaryrd}
\usepackage{mathdots}
\usepackage{float}
\usepackage{multirow}
\usepackage{here}
\usepackage{ae,aeguill}
\usepackage{fancyhdr}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{colordvi}
\usepackage{graphicx}
\usepackage{amsfonts}
%\usepackage[toc,page]{appendix} 
\usepackage{fancybox}
\usepackage{moreverb}
\usepackage{pgf}
\usepackage{tabularx}
\usepackage{tikz}
\usetikzlibrary{calc,automata,arrows,chains,matrix,positioning,scopes}
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Z}{{\mathbb Z}}     % Integers
\newcommand{\N}{{\mathbb N}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\newcommand{\inv}{^{-1}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}

\newcommand{\D}{\mathbf{D}}

\newcommand{\A}{\mathbf{A}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\L}{\mathbf{L}}


\newcommand{\V}{\mathbf{V}}

\newcommand{\FO}{\mathbf{FO}}
\newcommand{\MSO}{\mathbf{MSO}}
\newcommand{\BS}{\mathbf{{\mathcal B}\Sigma}}
\newcommand{\X}{\mathbf{X}}
%\newcommand{\LI}{\mathbf{LI}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\F}{\mathbf{F}}

\newcommand{\Sigun}{\Sigma_1[<]}

\newcommand{\T}{\mathbf{TL}}

\newcommand{\equations}[1]{{\llbracket #1\rrbracket}}

\newcommand{\clot}{\uparrow\!\!}
\newcommand{\clotb}{\downarrow\!\!}

\newcommand\nostarr[2]{\hspace{2pt}\raisebox{#1pt}{$#2$}\hspace{4pt}}
\newcommand\nostar[1]{\nostarr{2}{#1}}
\newcommand\withstarr[2]{\setbox3=\hbox{$*$}\hspace{-\wd3}
\hspace{-3pt}\raisebox{8pt}{\smash{$*$}}\nostarr{#1}{#2}}
\newcommand\withstar[1]{\withstarr{2}{#1}}

\newcommand{\tvi}{\vrule height 12pt depth 5 pt width 0 pt}

\newcommand{\lowtvi}{\vrule height 0pt depth 6 pt width 0 pt}

\newcommand{\ptvi}{\vrule height 10pt depth 4 pt width 0 pt}
\setlength{\fboxsep}{1.5pt}




\newcommand{\Bchap}{\widehat{\cA}'}
\newcommand{\LL}{\sim_{ll}}
\newcommand{\LR}{\sim_{lr}}
\newcommand{\RL}{\sim_{rl}}
\newcommand{\RR}{\sim_{rr}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cL}{\mathcal{L}}

%macros transition monoid
\newcommand{\ud}{$(1,\leftarrow)$}
\newcommand{\ug}{$(1,\rightarrow)$}
\newcommand{\dd}{$(2,\leftarrow)$}
\newcommand{\dg}{$(2,\rightarrow)$}
\newcommand{\td}{$(3,\leftarrow)$}
\newcommand{\tg}{$(3,\rightarrow)$}


\newsavebox{\Jclass}
\sbox{\Jclass}{
  \begin{tabular}{|c|c|}
  \hline
  \tvi $^*aba$ & $^*abb$ \\
  \hline
  \tvi $^*bba$ & $^*bb$ \\
  \hline
  \end{tabular}
  }
